Slapo: A Schedule Language for Progressive Optimization of Large Deep Learning Model Training

Recent years have seen an increase in the development of large deep learning (DL) models, which makes training efficiency crucial. Common practice is struggling with the trade-off between usability and performance. On one hand, DL frameworks such as PyTorch use dynamic graphs to facilitate model developers at a price of sub-optimal model training performance. On the other hand, practitioners propose various approaches to improving the training efficiency by sacrificing some of the flexibility, ranging from making the graph static for more thorough optimization (e.g., XLA) to customizing optimization towards large-scale distributed training (e.g., DeepSpeed and Megatron-LM). In this paper, we aim to address the tension between usability and training efficiency through separation of concerns. Inspired by DL compilers that decouple the platform-specific optimizations of a tensor-level operator from its arithmetic definition, this paper proposes a schedule language, Slapo, to decouple model execution from definition. Specifically, Slapo works on a PyTorch model and uses a set of schedule primitives to convert the model for common model training optimizations such as high-performance kernels, effective 3D parallelism, and efficient activation checkpointing. Compared to existing optimization solutions, Slapo progressively optimizes the model "as-needed" through high-level primitives, and thus preserving programmability and debuggability for users to a large extent. Our evaluation results show that by scheduling the existing hand-crafted optimizations in a systematic way using Slapo, we are able to improve training throughput by up to 2.92x on a single machine with 8 NVIDIA V100 GPUs, and by up to 1.41x on multiple machines with up to 64 GPUs, when compared to the out-of-the-box performance of DeepSpeed and Megatron-LM.

==> sections/5.1-sec-single-gpu.tex <==
\subsection{Evaluation on a Single GPU}
\label{sub:single_device_exp}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/exp/single_device_v100.pdf}
\caption{End-to-end throughput on a single NVIDIA V100 16GB GPU. $\times$ denotes unsupported implementations.}
\label{fig:single_v100}
\end{figure}

We first conduct end-to-end training efficiency evaluations on a single GPU to demonstrate that \Name is generally applicable to various model implementations.

\noindent\textbf{Systems.}
We use PyTorch Eager mode~\cite{paszke2019pytorch} as the baseline, which provides out-of-the-box performance.
If activation checkpointing is implemented in a model, we evaluate the performance with and without activation checkpointing, and report the better one.
When applicable, we also include the performance result with TorchScript~\cite{torchscript}, a commonly-used compiler framework in PyTorch, as another baseline.
Since PyTorch 1.12, TorchScript adopts nvFuser~\cite{nvfuser} as the operator fusion mechanism, and supports training workloads.
For \Name, we schedule models with efficient kernels, operator fusion, and activation checkpointing, and leverage the auto-tuner proposed in \S\ref{sec:autotune} to search for the best configuration.

\noindent\textbf{Results.}
% \cody{find out why WideResNet with TS outperforms Slapo.}
Fig.~\ref{fig:single_v100} shows the throughput of each configuration. In most cases, \Name can consistently improve the training throughput.
Compared to Eager mode, \Name achieves 1.05$\times$-2.11$\times$ speedup.
Even compared to TorchScript-optimized models, \Name still achieves 1.45$\times$ speedup on average.
This is mainly attributed to \Name employing the similar operator fusion but with more optimizations such as activation checkpointing and efficient custom kernels. 
Note that although \Name's fusion capability is limited by module boundaries for structure-preserving scheduling, most performance bottleneck subgraphs do not cross modules in training workloads.

Furthermore, \Name enables more optimization opportunities than TorchScript by progressive tracing.
For example, the GPT model implementation we adopted is GPT-Neo~\cite{gao2020pile} from the HuggingFace hub. This implementation, unfortunately, cannot be optimized by TorchScript due to its coding style, thus showing no results in Fig.~\ref{fig:single_v100}.
However, \Name allows us to selectively trace the FFN (Feed-Forward Network) module but not others, resulting in effective optimization. % modules where TorchScript is not supported, and use TorchScript to fuse the computation.

In addition, \Name tunes the ratio of activation checkpointing to maximize GPU memory utilization.
For example, after tuning the ratio of activation checkpointing in BERT, we only checkpoint 25\% of attention layers.
This brings another 1.06$\times$ speedup compared to checkpointing all layers.


% TorchScript
% From this experiment, we observe TorchScript has several limitations.
% First, TorchScript requires the model to be carefully implemented with necessary type hints and static control flow~\cite{torchscript}.
% However, even with special treatment with HuggingFace GPT~\cite{wolf2019huggingface}, TorchScript is still unable to trace the model due to \texttt{NoneType} keyword arguments~\cite{ts_none_kwargs}.
% By contract, \Name only invokes the tracer when needed, so can minimize the impact of changing a part of dynamic graph into static for optimization.
% Second, TorchScript cannot be applied with activation checkpointing.
% Since the IR is flattened in the traced model, original checkpoints attached to each module block are no longer available.
% The Transformer models % like BERT, RoBERTa, and T5
% may have better training throughput when enabling activation checkpoints as the batch size can be enlarged, while TorchScript loses this opportunity.
% On the contrary, \Name preserves the module hierarchy and can apply checkpoints to models that do not have inherent support (e.g., ALBERT, WideResNet).
% Other optimization techniques can still be applied to a the \Name checkpointed model.
% Third, the performance of TorchScript-optimized models are not predictable, and it may introduce extra overheads.
% For OPT and T5 models, the traced model cannot apply the same batch size as the vanilla model, thus reducing the performance.
% However, every optimization described by \Name are transparent to users, and can be easily switched off if an optimization has a negative effect on the model.

==> sections/5.6-fidelity.tex <==
\subsection{Fidelity}
Pre-training GPT for several K iterations and comparing the loss trend between Megatron and HF models.

For transformer-based models, we use Wikipedia-en~\cite{wikipedia} corpus as the training dataset, and the micro-batch size is selected based on the memory footprint.

As shown in Fig.~\ref{fig:fidelity}, \Name converges at the same rate with DeepSpeed.

==> sections/6-sec-limitations.tex <==
\section{Limitations}
\label{sec:limitations}

Our tracer is inherited from the base tracer of \fx but adds support for control flow and hierarchical representation.
However, the control flow support is highly constrained by the random input data.
For one thing, we need advanced support for the constant propagation of the metadata.
We need to overload all the operators of the proxy to make sure the metadata can go through different modules.
For another, each time the tracer will only choose one path to execute and ignore others, which means if some features of the input data are dynamically changed (e.g., dynamic shapes), the traced model can only work for that specific kind of input.
We will need a quick transformation technique in order to trace and optimize the model just-in-time, so that it can suit different input data.

The functionality of the verifier is also limited.
Currently, we mainly depend on a large amount of randomly generated input data and test whether the output of the new module is the same as the original one.
However, it cannot work for a complex module with different branches.
Sampling-based verification cannot figure out whether the module is semantically correct.
In the future, we can incorporate symbolic shape propagation for the verifier instead of random inputs, so that we can further test if the shapes of the tensors match in the dataflow.

% Lastly, the auto-tuner is also limited.
% Although we have represented the schedule space with our proposed primitives, currently we only tune the checkpointing ratio for better memory usage.
% Actually, we can tune more primitives in the future, which provides more opportunities for optimizing distributed training for large models.
% Specifically, we can tune the number of devices used in 3D parallelism.
% We can also find the best kernel implementation for module replacement given a set of available kernels~\cite{jeon2022collage}.
